Morse moves in flow categories

We pursue the analogy of a framed flow category with the flow data of a Morse function. In classical Morse theory, Morse functions can sometimes be locally altered and simplified by the Morse moves. These moves include the Whitney trick which removes two oppositely framed flowlines between critical points of adjacent index and handle cancellation which removes two critical points connected by a single flowline. A framed flow category is a way of encoding flow data such as that which may arise from the flowlines of a Morse function or of a Floer functional. The Cohen-Jones-Segal construction associates a stable homotopy type to a framed flow category whose cohomology is designed to recover the corresponding Morse or Floer cohomology. We obtain analogues of the Whitney trick and of handle cancellation for framed flow categories: in this new setting these are moves that can be performed to simplify a framed flow category without changing the associated stable homotopy type. These moves often enable one to compute by hand the stable homotopy type associated to a framed flow category. We apply this in the setting of the Lipshitz-Sarkar stable homotopy type (corresponding to Khovanov cohomology) and the stable homotopy type of a matched diagram due to the authors (corresponding to sl_n Khovanov-Rozansky cohomology).

==> trefoils.tex <==
Let us consider the disjoint union of two (right-handed) trefoils, denoted $L$.
\begin{figure}[ht]
 \includegraphics[width=3cm,height=2cm]{fig_tref}\hspace{0.3cm}\includegraphics[width=3cm,height=2cm]{fig_tref}
\caption{The disjoint union of two trefoil knots.}
\end{figure}

The stable homotopy type of this link is easily derived from the stable homotopy type of the trefoil using \cite[Thm.1]{LawLipSar}. Also, the stable homotopy type of the trefoil $T$ is just a wedge of Moore spaces determined by the Khovanov homology, but it is also easily derived from the diagram using one elementary tangle of index 3 and \cite[Thm.1.2]{JLS}. In fact, the sock flow category is
\[
 \begin{array}{ccccccc}
  \includegraphics[width=1cm, height=0.6cm]{fig_tref0} & \stackrel{+}{\longleftarrow} & \includegraphics[width=1cm, height=0.6cm]{fig_tref1} & \stackrel{+-}{\longleftarrow} & \includegraphics[width=1cm, height=0.6cm]{fig_tref1} & \stackrel{++}{\longleftarrow} & \includegraphics[width=1cm, height=0.6cm]{fig_tref1}\\
 0 & & 1 & & 2 & & 3
 \end{array}
\]
In quantum degree $q=7$ we only get two objects, the circle above $2$ with a $+$ label and the circle above $3$ with a $-$ label, and $2$ positively framed points between them. In particular,
\[
 \X^\Kh_7(T) \simeq M(\Z/2,2).
\]
By \cite[Thm.1]{LawLipSar} $\X^\Kh_{14}(L)$ contains $M(\Z/2,2)\wedge M(\Z/2,2)$ as a wedge summand, an elementary Chang complex (see \cite[\S 11]{baues}) and not decomposable into Moore spaces. Nevertheless, let us consider the flow category $\cL^\Kh_{14}(L_{(3,3)})$. There are in fact only $6$ objects, depicted in Figure \ref{fig_flowcattrefs}.
\begin{figure}[ht]
\begin{tikzpicture}
 \node at (0,0) {$\stackrel{\includegraphics[width=0.8cm]{fig_tref1}^-\includegraphics[width=0.8cm]{fig_tref1}^-}{(3,3)}$};
 \node at (-5,-2) {$\stackrel{\includegraphics[width=0.8cm]{fig_tref1}^-\includegraphics[width=0.8cm]{fig_tref1}^+}{(2,3)}$};
 \node at (-2,-2) {$\stackrel{\includegraphics[width=0.8cm]{fig_tref1}^+\includegraphics[width=0.8cm]{fig_tref1}^-}{(2,3)}$}; 
 \node at (5,-2) {$\stackrel{\includegraphics[width=0.8cm]{fig_tref1}^+\includegraphics[width=0.8cm]{fig_tref1}^-}{(3,2)}$};
 \node at (2,-2) {$\stackrel{\includegraphics[width=0.8cm]{fig_tref1}^-\includegraphics[width=0.8cm]{fig_tref1}^+}{(3,2)}$};
 \node at (0,-4) {$\stackrel{\includegraphics[width=0.8cm]{fig_tref1}^+\includegraphics[width=0.8cm]{fig_tref1}^+}{(2,2)}$};

 \draw [shorten >=0.8cm,shorten <=0.4cm,->] (0,-0.4) -- node [above] {$++$} (-2.5,-1.8);
 \draw [shorten >=0.8cm,shorten <=0.4cm,->] (0,-0.4) -- node [above] {$--$} (2.5,-1.8);
 \draw [shorten >=0.8cm,shorten <=0.4cm,<-] (0,-3.6) -- node [above] {$++$} (-2.5,-2.2);
 \draw [shorten >=0.8cm,shorten <=0.4cm,<-] (0,-3.6) -- node [above] {$++$} (2.5,-2.2);
\end{tikzpicture}
\caption{The flow category $\cL^\Kh_{14}(L_{(3,3)})$.}
\label{fig_flowcattrefs}
\end{figure}

Notice that the outside objects in the middle row are isolated from all other objects. This means they contribute two copies of $S^5$ to the stable homotopy type. To describe the $1$-dimensional moduli spaces, let us introduce more notation. We call the top object $\gamma$, the bottom object $\alpha$ the middle objects $\beta_1$ and $\beta_2$ where $\beta_1$ is based at $(2,3)$ while $\beta_2$ is based at $(3,2)$. Write 
\begin{align*}
\M(\gamma,\beta_1) &= \{P_0,P_1\} &  \M(\gamma,\beta_2) = \{\tilde{P}_0,\tilde{P}_1\} \\
\M(\beta_1,\alpha) &= \{p_0,p_1\} &  \M(\beta_2,\alpha) = \{\tilde{p}_0,\tilde{p}_1\}.
\end{align*}
Following \cite[\S 5.2]{JLS}, we get four intervals in $\M(\gamma,\alpha)$ as follows:

\begin{tikzpicture}
\node[label=below:$p_0\,P_0$, label=above:{\color{blue}$\beta_1$}] (5_5_1)at (0,0) {};
\node[label=below:$\tilde{p}_0\,\tilde{P}_0$, label=above:{\color{blue}$\beta_2$}] (5_5_2)at (1.6,0) {};

\draw[|-|] (5_5_1)--(5_5_2);

\node[label=below:$p_0\,P_1$, label=above:{\color{blue}$\beta_1$}] (5_5_3)at (3.3,0) {};
\node[label=below:$\tilde{p}_1\,\tilde{P}_0$, label=above:{\color{blue}$\beta_2$}] (5_5_4)at (4.9,0) {};

\draw[|-|] (5_5_3)--(5_5_4);

\node[label=below:$p_1\,P_0$, label=above:{\color{blue}$\beta_1$}] (5_5_5)at (6.6,0) {};
\node[label=below:$\tilde{p}_0\,\tilde{P}_1$, label=above:{\color{blue}$\beta_2$}] (5_5_6)at (8.2,0) {};

\draw[|-|] (5_5_5)--(5_5_6);

\node[label=below:$p_1\,P_1$, label=above:{\color{blue}$\beta_1$}] (5_5_7)at (9.9,0) {};
\node[label=below:$\tilde{p}_1\,\tilde{P}_1$, label=above:{\color{blue}$\beta_2$}] (5_5_8)at (11.5,0) {};

\draw[|-|] (5_5_7)--(5_5_8);
\end{tikzpicture}

Since $\alpha$ is based at $(2,2)$ and all four intervals correspond to a $(P,P)$-cell in the obstruction complex (see \cite[\S 5.2]{JLS}), all intervals are framed $0$. We cannot perform a Whitney trick or a handle cancellation directly, but consider the flow category $\Cat$ depicted in Figure \ref{fig_supcat}.

\begin{figure}[ht]
 \begin{tikzpicture}[scale =1,
roundnode/.style={circle, draw=black!, very thick}
]
%Nodes
\draw [very thick] (-3,0) circle [radius=0.3];
\draw [very thick] (3,0) circle [radius=0.3];
\draw [very thick] (-3,-2) circle [radius=0.3];
\draw [very thick] (0,-2) circle [radius=0.3];
\draw [very thick] (3,-2) circle [radius=0.3];
\draw [very thick] (0,-4) circle [radius=0.3];

\node at (-3,0) {$\gamma$};
\node at (3,0) {$\tau$};
\node at (-3,-2) {$\beta_1$};
\node at (0,-2) {$\beta_2$};
\node at (3,-2) {$\sigma$};
\node at (0,-4) {$\alpha$};

\draw [->, shorten >=0.4cm, shorten <=0.4cm] (-3,0)--(-3,-2) node[sloped,below,pos=0.4]{$P_0\,P_1$};
\draw [->, shorten >=0.4cm, shorten <=0.4cm] (-3,0)--(0,-2) node[sloped,above,pos=0.3]{$\tilde{P}_0\,\tilde{P}_1$};
\draw [->, shorten >=0.4cm, shorten <=0.4cm, gray] (3,0)--(-3,-2) node[sloped,above,pos=0.3]{$-$};
\draw [->, shorten >=0.4cm, shorten <=0.4cm, gray] (3,0)--(0,-2) node[sloped,above,pos=0.7]{$+$};
\draw [->, shorten >=0.4cm, shorten <=0.4cm, gray] (3,0)--(3,-2) node[sloped,above,pos=0.3]{$+$};
\draw [->, shorten >=0.4cm, shorten <=0.4cm] (-3,-2)--(0,-4) node[sloped,below,pos=0.4]{$p_0\,p_1$};
\draw [->, shorten >=0.4cm, shorten <=0.4cm] (0,-2)--(0,-4) node[sloped,above,pos=0.5]{$\tilde{p}_0\,\tilde{p}_1$};
\end{tikzpicture}
\caption{The flow category $\Cat$.}
\label{fig_supcat}
\end{figure}
The moduli space $\M(\gamma,\alpha)$ is as in $\cL^\Kh_{14}(L_{(3,3)})$, and $\M(\tau,\alpha)$ is given by two intervals
\[
\begin{tikzpicture}
\node[] at (-1.5,0) {$\mathcal{M}(\tau,\alpha) =$};
\node[label=below:$p_0\,-$, label=above:{\color{blue}$\beta_1$}] (5_5_1)at (0,0) {};
\node[label=below:$\tilde{p}_1\,+$, label=above:{\color{blue}$\beta_1$}] (5_5_2)at (1.6,0) {};
\node[label=below:$p_1\,-$, label=above:{\color{blue}$\beta_1$}] (5_5_3)at (3.3,0) {};
\node[label=below:$\tilde{p}_0\,+$, label=above:{\color{blue}$\beta_1$}] (5_5_4)at (4.9,0) {};

\node[] at (2.4,0) {$\cup$};

\draw[|-|] (5_5_3)--(5_5_4) node[sloped, above,pos=0.5, red]{$\varepsilon_2$};
\draw[|-|] (5_5_1)--(5_5_2) node[sloped, above,pos=0.5, red]{$\varepsilon_1$};
\end{tikzpicture}
\]
for some $\varepsilon_1,\varepsilon_2\in \Z/2$. 

If we cancel the pair $\tau,\sigma$ we obtain the relevant part of the flow category $\cL^\Kh_{14}(L)$. But if we cancel the pair $\tau,\beta_2$ we get the flow category $\overline{\Cat}$ given in Figure \ref{fig_supcatcan}.

\begin{figure}[ht]
 \begin{tikzpicture}[scale =1,
roundnode/.style={circle, draw=black!, very thick}
]
%Nodes
\draw [very thick] (0,0) circle [radius=0.3];
\draw [very thick] (-3,-2) circle [radius=0.3];
\draw [very thick] (3,-2) circle [radius=0.3];
\draw [very thick] (0,-4) circle [radius=0.3];

\node at (0,0) {$\bar{\gamma}$};
\node at (-3,-2) {$\bar{\beta_1}$};
\node at (3,-2) {$\bar{\sigma}$};
\node at (0,-4) {$\bar{\alpha}$};

\draw [->, shorten >=0.4cm, shorten <=0.4cm] (0,0)--(-3,-2) node[sloped,above,pos=0.5]{$P_0\,P_1\, M_0\,M_1$};
\draw [->, shorten >=0.4cm, shorten <=0.4cm] (0,0)--(3,-2) node[sloped,above,pos=0.3]{$\hat{P}_0\,\hat{P}_1$};
\draw [->, shorten >=0.4cm, shorten <=0.4cm] (-3,-2)--(0,-4) node[sloped,below,pos=0.4]{$p_0\,p_1$};
\end{tikzpicture}
\caption{The flow category $\overline{\Cat}$.}
\label{fig_supcatcan}
\end{figure}

We denote the new points in $\M(\bar{\gamma},\bar{\beta_1})$ by $M_0 = (-,\tilde{P}_0)$ and $M_1=(-,\tilde{P}_1)$, and both are framed negatively.
Using Proposition \ref{prop:gluing_form_ii}(5) we get that $\M(\bar{\gamma},\bar{\alpha})$ still consists of $4$ intervals given by

\begin{tikzpicture}
\node[label=below:$p_0\,P_0$, label=above:{\color{blue}$\beta_1$}] (5_5_1)at (0,0) {};
\node[label=below:$p_1\,M_0$, label=above:{\color{blue}$\beta_1$}] (5_5_2)at (1.6,0) {};

\draw[|-|] (5_5_1)--(5_5_2) node[sloped, above,pos=0.5, red]{$\varepsilon_2$};

\node[label=below:$p_0\,P_1$, label=above:{\color{blue}$\beta_1$}] (5_5_3)at (3.3,0) {};
\node[label=below:$p_0\,M_0$, label=above:{\color{blue}$\beta_2$}] (5_5_4)at (4.9,0) {};

\draw[|-|] (5_5_3)--(5_5_4) node[sloped, above,pos=0.5, red]{$\varepsilon_1$};

\node[label=below:$p_1\,P_0$, label=above:{\color{blue}$\beta_1$}] (5_5_5)at (6.6,0) {};
\node[label=below:$p_1\,M_1$, label=above:{\color{blue}$\beta_2$}] (5_5_6)at (8.2,0) {};

\draw[|-|] (5_5_5)--(5_5_6) node[sloped, above,pos=0.5, red]{$\varepsilon_2$};

\node[label=below:$p_1\,P_1$, label=above:{\color{blue}$\beta_1$}] (5_5_7)at (9.9,0) {};
\node[label=below:$p_0\,M_1$, label=above:{\color{blue}$\beta_2$}] (5_5_8)at (11.5,0) {};

\draw[|-|] (5_5_7)--(5_5_8) node[sloped, above,pos=0.5, red]{$\varepsilon_1$};
\end{tikzpicture}

After performing the Whitney trick with $P_0,M_0$ and using Proposition \ref{

\[
 \X^\Kh_{14}(L) \simeq \Sigma^2 (\RP^2\wedge \RP^2) \vee S^5 \vee S^5,
\]
a result we can also read off directly from \cite[Thm.1]{LawLipSar}.

\begin{remark}
 While we cannot perform a Whitney trick or a handle cancellation, one can do a handle slide on $\cL^\Kh_{14}(L_{(3,3)})$ followed by several Whitney tricks to turn this flow category into one that can be easily identified as a standard Chang complex in the sense of \cite[\S 11]{baues}. We will give the construction of a handle slide on a framed flow category in an upcoming paper.
\end{remark}


% \[
%  \xymatrix@!=1.5pc{ & & \includegraphics[width=0.8cm]{fig_tref1}^-\includegraphics[width=0.8cm]{fig_tref1}^- \ar[lld] \ar[rrd] \\
% \stackrel{\includegraphics[width=0.8cm]{fig_tref1}^-\includegraphics[width=0.8cm]{fig_tref1}^+}{(2,3)} & 
% \stackrel{\includegraphics[width=0.8cm]{fig_tref1}^-\includegraphics[width=0.8cm]{fig_tref1}^+}{(2,3)} & & (3,2) & (3,2)}
% \]

